Distributed Parameter Estimation in Probabilistic Graphical Models

This paper presents foundational theoretical results on distributed parameter estimation for undirected probabilistic graphical models. It introduces a general condition on composite likelihood decompositions of these models which guarantees the global consistency of distributed estimators, provided the local estimators are consistent.

==> compositelikelihood.tex <==

\section{Generalisation to distributed composite-likelihood}
\label{sec:cl}

We ended Section~\ref{sec:background} questioning the conditions under which the simple consensus estimators of Liu and Ihler \cite{Liu:2012} are consistent. In particular, under what conditions does Equation~(\ref{eq:a}) apply?

In Section~\ref{sec:clap}, we showed that as long we use normalized potential representation for the joint and conditionals, Equation~(\ref{eq:a}) holds true and, hence, all the consistency and asymptotic normality results of Liu and Ihler hold true.

We should note that the conditional distributions in Section~\ref{sec:clap} are over single (or several) cliques. We are therefore in the more general setting of conditional composite-likelihood. Armed with the CLAP argument and the consistency of CLAP, it is trivial to generalise the M-estimation theorems of Liu and Ihler to consensus conditional composite-likelihood estimators. 

Likewise, the results of Section~\ref{sec:lap} enable us to generalise the M-estimation theorems of Liu and Ihler to consensus marginal composite-likelihood estimators. 

While it is enough to use LAP or CLAP estimators to obtain consistent estimators of the parameters of the joint distribution, it may be the case that applying the consensus criteria (for example, averaging parameters of each auxiliary MRF as in Liu and Ihler) results in more efficient estimators. Our experiments in the following section analyse this question. 

We should add that the LAP and CLAP estimators require less communication than the consensus or full-composite likelihood estimators. Hence, they should be preferred in settings such as remote sensing, where communication is very expensive or prone to transmission errors.


==> experiments.tex <==

\section{Experiments}
\label{sec:pl}

LAP and CLAP are fully parallel and hence have lower communication cost than the consensus and centralized estimators. The local estimators (auxiliary MRFs) involves similar computational costs. While the questions of communication and computation costs is clear, it is less clear which estimators are more statistically efficient. For this reason, we focus on the latter question in our empirical analysis.


In the experiments, we compare the following estimators:
\begin{enumerate}
\item LAP with $\fq$ and $\fq^{\tiny 1 node}$ clique neighbourhoods.
\item CLAP.
\item Centralised conditional CL.
\item Centralised marginal CL by products of auxiliary MRFs. (2 versions: with and without added edges in auxiliary MRFs)
\item Linear-consensus CLAP and LAP (3 methods)
\item Max-consensus CLAP and LAP (3 methods)
\end{enumerate}

Repeat the above for grid MRF, fully observed RBM (when applicable), others from ICML paper depending on time.


==> pseudolikelihood.tex <==

\section{Distributed parameter estimation via pseudo-likelihood}
\label{sec:pl}

- Ihler: Distributed pseudo-likelihood, and some very general claims.
- There's a problem with these claims: The assumptions don't hold in the general case.


